From Stream to Pool: Pricing Under the Law of Diminishing Marginal Utility

Dynamic pricing models often posit that a $\textbf{stream}$ of customer interactions occur sequentially, where customers' valuations are drawn independently. However, this model is not entirely reflective of the real world, as it overlooks a critical aspect, the law of diminishing marginal utility, which states that a customer's marginal utility from each additional unit declines. This causes the valuation distribution to shift towards the lower end, which is not captured by the stream model. This motivates us to study a pool-based model, where a $\textbf{pool}$ of customers repeatedly interacts with a monopolist seller, each of whose valuation diminishes in the number of purchases made according to a discount function. In particular, when the discount function is constant, our pool model recovers the stream model. We focus on the most fundamental special case, where a customer's valuation becomes zero once a purchase is made. Given $k$ prices, we present a non-adaptive, detail-free (i.e., does not "know" the valuations) policy that achieves a $1/k$ competitive ratio, which is optimal among non-adaptive policies. Furthermore, based on a novel debiasing technique, we propose an adaptive learn-then-earn policy with a $\tilde O(k^{2/3} n^{2/3})$ regret.

==> OR/Learning.tex <==
%%%%% New attempt at writing this, Old version \iffalse'd below

Now we consider adaptive policies in the presence of unknown demand.  Specifically, {\new the seller only knows that the underlying \ins\ $\cal I$ comes from the family ${\cal F}(\lam,{\cal P},n)$ of instances with interaction rate $\lam$, price set $\cal P$ and a total number $n$ of customers.
%\footnote{It is enough to have a good estimate of $n$, say within $XXX$ additive error. \textcolor{red}{TODO: Analyze what happens when $n$ is mis-specified and fill in something for XXX.}}
% the , and the interaction rate $\lambda$, but not 
In \parti, the seller does not know the number $n_j$ of customers with valuation $p_j$.
% Our policies aim to simultaneously learn the demand and optimize  pricing decisions given a finite time horizon.  
% As is standard in the literature, 
We will analyze the \emph{regret} of our policy against ${\rm OPT}_{\rm NA} ({\cal I})$, the expected revenue of an optimal non-adaptive policy.
%Where it is clear, we use $\opt(\cI)$ instead of ${\rm OPT}_{\rm NA} ({\cal I})$ in this section.
We abuse notation slightly and use $\opt(\cI)$ instead of ${\rm OPT}_{\rm NA} ({\cal I})$ in this section.

%which measures the difference in revenue of the proposed policy to the best policy in a class $\Pi$ of \emph{benchmark policies}, which are usually equipped with additional information not available to our policy.  
%As before, we consider the worst case regret against a family of demand functions $\mathcal{F}$.  This leads to the following definition.
% Thus we define the worst-case regret as follows.

\begin{definition}[Regret]
For any UDPM \ins\ ${\cal I} = {\rm UDPM}(\lambda, {\cal P}, (n_j)_{j \in[k]})$, we define the {\em regret} of a policy $\pi$ as 
$\textrm{Regret}(\pi, \cal{I}) := \left\{ {\rm OPT}({\cal I}) - {\rm Rev}(\pi,{\cal I}) \right\}$.
    % where the supremum is taken over all instances ${\cal I}$ where the total number of customers is $n$, the price levels are given by ${\cal P}$, and the interaction rate is $\lambda$.
    % The numbers $n_j$ may vary arbitrarily subject to the constraint $\sum_{j \in [k]} n_j = n$.
\end{definition}
}

As the main result of this section, we present an \adap\ detail-free policy with sublinear regret in {\bf both} $n$ and $k$.  
Our {\em learn-then-earn} (LTE) policy first learns $n_j$'s by exploring each price, then commits to an optimal non-adaptive policy for the learned instance in the remainder of the time horizon.  
While this is similar to the {\em Explore-Then-Commit} (ETC) algorithm for MAB, we will see that there are several new challenges in the analysis.

\begin{theorem}[Adaptive Policy with Sublinear Regret]
\label{thm:regret_bound}
{\new For any $\lam, {\cal P}, n$, there exist parameters for \cref{alg:learn_then_earn} such that for any
${\cal I}\in {\cal F}(\lam, {\cal P}, n)$, we have
${\rm Regret}(\pi^{\rm LTE}, {\cal I}) = \tilde O(p_1 (kn)^{2/3})$.} 
\end{theorem}

% \tl{The analysis holds as long as $\lambda$ is known and $\lambda s \leq 1.59$.  This is true as long as $n$ is large enough for our choice of $s = \lambda^{-1} (kn)^{-1/3}$.  For me this is enough to not worry about dependence on $\lambda$.}
% \su{Check: whether the analysis holds for general $\lambda$ (instead of just $\lambda = \Theta(1)$.  If so, then let's specify $\lambda$ in the regret bounds.}

Our regret bound is higher than the minimax optimal $\tilde \Theta(\sqrt{kn})$ regret \citep{auer2002finite} for the stream model (which is equivalent to $k$-armed bandits). 
Intuitively, this is because in the stream model, the effect of exploration is {\bf local} in the sense that what the seller's decisions in any time interval only affects the customers arriving in that interval.
{\new In contrast, the effect of any decision in our model is {\bf global}: A poor choice of price can potentially affect $\Omg(n)$ customers.  
Thus, it is reasonable to expect a higher regret in the pool model.}

Our policy is formally described below in \cref{alg:learn_then_earn}.
The policy operates in two phases. 
Initially, we explore each of the price levels $p_1,p_2,\ldots, p_{k}$ for fixed intervals of length $s_1,s_2,\ldots, s_{k}$. 
After exploring each price $p_j\in \cal P$, we construct an estimate $\widehat n_j$ of $n_j$ using the realized demand $D_1,\dots,D_j$, {\new based on a novel debiasing approach which we will explain in \cref{sec:debias}.}

We then compute an optimal non-adaptive  policy for the estimated instance $\widehat {\cal I} = 
(\lambda, {\cal P}, \{\widehat n_j\}_{j \in [k]})$
%(T d- \sum_i s_i, n-\sum_{i < k} D_i, \{\widehat n_i\}_{i=1}^k, \{ v_i\}_{i=1}^k, \lambda)$ 
using only the shortened horizon of length $1-s_{\rm total}$, where $s_{\rm total} = \sum_{j=1}^k s_j$ is the total exploration time. 
{\new This can be done efficiently using the dynamic program in \cref{thm:optimal_non_adap}.}
% Following this policy for the remaining time constitutes a feasible policy overall.

%In order to show that this policy has low regret, first we must show that we may take $s_1,s_2,\ldots,s_{k-1}$ small enough so that the exploration period incurs low regret.  Next, we need to show that the estimates $\{\widehat n_i\}_{i=1}^k$ are good enough so that the optimal policy on the ``pseudo-instance'' $\widehat {\cal I}$ gives us close to the optimal revenue in expectation.  To demonstrate the key ideas in our analysis, in the next section we first restrict to the case of $k=2$ different price levels.

\begin{algorithm}
\caption{Learn-then-Earn Policy \label{alg:learn_then_earn}}
%\LinesNumbered
\DontPrintSemicolon
\SetKwComment{Comment}{//}{}
\KwData{Partial Instance  $(\lambda, {\cal P}, n)$, \ Exploration times $(s_1, s_2, \ldots, s_{k})$}
\KwResult{Policy $\pi^{\rm LTE}$}

\Comment*[l]{Learning phase}
\For{$j = 1,2,\ldots, k$}{
Select $p_j$ for time $s_j$ and observe sales $D_j$
}
%\Comment*[l]{Construct estimates $\{\widehat n_j\}_{j=1}^k$}

Define the function $q(x) = 1-\exp(-\lambda x)$

\For{$j=1,2,\ldots,k$}{
$\widehat n_j \gets \frac{D_j}{q(s_j)} - \sum_{i\le j-1} (\widehat n_i - D_i)$
}

\Comment*[l]{Earning Phase}
%$\widehat \cI \gets (T-\sum_{i < k} s_i, n, \{\widehat n_i\}_{i=1}^k, \{v_i\}_{i=1}^k, \lambda)$
$\widehat {\cal I} \gets
{\rm UDPM}\lb(\lambda, {\cal P}, \{\widehat n_j\}_{j \in [k]}\rb)$

$s_{\rm total} \gets \sum_{j=1}^{k} s_j$

%Compute an optimal non-adaptive policy $\widehat t_1,\ldots, \widehat t_k$ for the instance $\widehat \cI$
Find optimal non-adaptive policy $\widehat{\bf t} = (\widehat t_j)_{j \in [k]}$ for $\widehat \cI$ on the time interval $[0, 1- s_{\rm total}]$

\For{$j=1,2,\ldots,k$}{
Select price $p_j$ in $[\widehat t_j + s_{\rm total}, \widehat t_{j+1} + s_{\rm total}]$
}
\end{algorithm}

% \su{Add a remark to explain why existing results for adv bandits do. Need to read Slivkins et al FOCS'2020 paper on adv bandits with Knapsack. Also read Even-Dar, Mansour, MOOR'09 paper on adv MDP.}

\subsection{Debiasing the Demand} \label{sec:debias}
As is standard in MAB, we aim to construct \emph{unbiased} estimates of the model parameters. 
In Algorithm \ref{alg:learn_then_earn}, we use price $p_1$ in the time interval $[0,s_1]$ and track the (random) demand $D_1$ during this period. 
Recall that each customer monitors the price with Poisson rate $\lambda$, so  $D_1 \sim {\rm Binomial}(n_1, q(s_1))$ where $q(x) := 1-\exp(-\lambda x)$. 
Thus, $D_1 / q(s_1)$ is an unbiased estimate of $n_1$.

However, when we explore lower prices, the situation is more complicated.  
There may still be active customers (i.e., customers who have not exited the market) with a valuation $p_1$ that purchase during this time, {\bf confounding} the future demands $D_2, D_3, \ldots, D_k$.

As a pivotal step, we develop a novel unbiased estimator to overcome this. 
Starting with $\widehat n_1 = D_1 / q(s_1)$, for each $j =2,3,\dots, k$, we recursively define 
\begin{equation} \label{eqn:estimates}
   \widehat n_j = \frac{D_j}{q(s_j)} - \sum_{i\le j-1}(\widehat n_i - D_i),
\end{equation}
The first part is similar to the naive estimator for $\widehat n_1$, while the second part aims to {\new ``de-confound'' the signals from  customers with higher valuations. }
We show that this estimator is unbiased.

\begin{lemma}[Unbiasedness] \label{lem:unbiased_estimates}
For any UDPM \ins\ ${\cal I}$ and \alg\ \pmt s $s_1, s_2, \ldots, s_{k}$, 
% be the lengths of each exploration period and $D_1,D_2,\ldots,D_{k}$ be the realized demands.  
we have $\ho{E} [\widehat n_j] = n_j$ for any $j=1,\dots,k$.
\end{lemma}

The above follows by induction on $j$.
The base case holds \triv ly.  
For the inductive case $1 < j \leq k$, we observe that conditioned on $D_i$ for $i < j$, we have $D_j \sim {\rm Bin}\lb(\sum_{i \leq j} n_i - \sum_{i\le j-1} D_i,\  q(s_j)\rb).$  
% Thus, \[\ho{E}[D_i] = \ho{E}\lb[\lb(n_i + \sum_{j\le i-1} n_j - \sum_{j\le i-1} D_j\rb)q\rb]= n_i q + \sum_{j\le i-1}\ho{E}[n_j - D_j].\]
Taking the expectation of our estimator $\hat n_j$ conditioned on $D_i$ for $i < j$, we have
\[ \ho{E}[\widehat n_j \mid D_1,D_2,\ldots ,D_{j-1}] = \sum_{i \leq j} n_j - \sum_{i \leq j-1} D_i - \sum_{i \leq j-1} (\widehat n_i - D_i) = n_j +  \sum_{i \leq j-1} \lb(n_i - \widehat n_i\rb),\]
where the first equality follows from the definition of $\widehat n_j$ in \cref{eqn:estimates} and that $D_j$ has a binomial distribution when conditioned on $D_1,D_2, \ldots, D_{j-1}$. 
The statement follows by (i) taking the expectation over $D_1,D_2,\ldots ,D_{j-1}$,  (ii) applying the induction hypothesis and (iii) applying the tower rule.

\iffalse
\proof
    We proceed by induction on $i < k$.  
    For the base case $i=1$, recall that $D_1 \sim {\rm Binom}(n_1 ,q(s_1))$.  Thus
    \[
    \E[ \widehat n_1] = \frac{1}{q(s_1)} \E[D_1] = n_1.
    \]
    Now for $1 < i < k$, we assume for induction that $\widehat n_j$ is unbiased for $j < i$.  
    Conditional on $D_j$ for $j < i$, it can be seen that $D_i \sim {\rm Binomial}(\sum_{j \leq i }n_j - \sum_{j < i} D_j, q(s_i))$. 
    This is because all customers with valuations $v_j$ for $j \leq i$ are active at this point but $\sum_{j < i} D_j$ such customers have left the market in earlier phases.  Now we have
    \[ \begin{split}
         \E[\widehat n_i \mid \{D_j\}_{j < i}]  =&  \frac{1}{q(s_i)}\E[D_i \mid \{D_j\}_{j < i} ] \\
         &- \sum_{j < i}(\widehat n_j - D_j) \\
         =& \sum_{i\leq j} n_j - \sum_{j < i} D_j - \sum_{j < i}(\widehat n_j - D_j) \\
         =& n_i + \sum_{j < i}(n_j - \widehat n_j)
    \end{split} 
    \]
    Now using the inductive hypothesis, we have
    \[
    \E[ \widehat n_i] =\E[\E[\widehat n_i \mid \{D_j\}_{j < i}]] = n_i + \sum_{j < i} \E[n_j - \widehat n_j] = n_i
    \]
    Finally, using the unbiasedness of $\widehat n_i$ for $i < k$, we have
    \[
    \E[\widehat n_k] = n - \sum_{i <k} \E[\widehat n_i] = n- \sum_{i <k} n_i = n_k,
    \]
    completing the proof.
\endproof

\fi


\subsection{Warm-up: The Two-Price Setting} \label{sec:two_price_case}

We demonstrate the main ideas by showing a regret bound of $\tilde{O}(n^{2/3})$ when $k=2$. 
% When there are only $k=2$ price levels $v_1 > v_2$, our proposed policy simplifies greatly.  
Consider the following simplified version of Algorithm~\ref{alg:learn_then_earn} for two price levels.
% \tl{Putting the previous sentence because Algorithm~\ref{alg:learn_then_earn} changed slightly.}
% Su: OK
We specify an exploration time $s \in [0,1]$, then set the price $X_t = p_1$ for all $t \leq s$. 
Let $D_1$ be the demand observed in this period.  
As discussed in \cref{sec:debias}, we use $\widehat n_1 = D_1/ q(s)$ and $\widehat n_2 = n - \widehat n_1$ as unbiased estimates of $n_1$ and $n_2$.  
Using these, we construct the estimated instance $\widehat {\cal I} = (\lambda, {\cal P}, (\widehat n_1, \widehat n_2))$.
%$(T-s, n - D, \{\widehat n_1 - D, \widehat n_2 \},\{v_1, v_2\} ,\lambda))$ 
and compute a non-adaptive policy $\widehat \pi$ achieving revenue ${\rm OPT}(\widehat {\cal I})$ for the remaining time horizon $1-s$ and commit to it.

\iffalse
{\color{blue} (Proof sketch)
choose the exploration period to be $n^{-1/4}$.
We then show that this results in an estimation $\widehat n_1,\widehat n_2$ such that \[|n_1 - \widehat n_1| \le n^{3/4}.\]
To see this, note that the observed demand at the end of the exploration period follows a Binomial \distr\ ${\rm Bin}(n_1,1-e^{-\lambda s})$. 
By Taylor expansion, for small $s$ we have $1-e^{-\lambda s} \sim q(s):=\lambda s$. 
Applying standard concentration bounds to ${\rm Bin}(n_1, q)$, we obtain \[|n_1 - \widehat n_1| \le \frac {\sqrt n}q\] with \prb\ $n^{-10}$.
The $n^{3/4}$ error then immediately follows by choosing $s=n^{-1/4}$.
}
\fi

\iffalse
Our goal is to show that the worst-case regret of this policy is $\tilde O(n^{3/4})$.  This policy incurs regret in a few ways.  One way we incur regret is due to exploration and using a smaller time horizon for the pseudo-instance.  Another way we incur regret is due to estimation error in $\widehat n_1$ and $\widehat n_2$ affecting the revenue we get in the ``earning'' phase of the algorithm.  We will show that both of these contributions are small.
\fi


\iffalse
Proceeding with the formal analysis,  we first define and characterize the expected revenue of an optimal non-adaptive policy.

\su{Note: possibly we need to move this up front, to Section 2}
\begin{definition} \label{def:rev_two_price}
    For $s \in [0,T]$ let $R(s; {\cal I})$ be the expected revenue of the non-adaptive policy which uses price $v_1$ for $s$ steps then price $v_2$ for $T-s$ steps on instance ${\cal I} = (T,n, \{n_1,n_2\}, \{v_1, v_2\}, \lambda)$.
\end{definition}
\su{Lower bound analysis also uses this result}

We have the following clsoed-form formula for the expected revenue. Recall that $q(s) = 1- \exp(-\lambda s)$.
\begin{proposition}[Optimal Revenue] \label{prop:opt_rev_two_price}
% \su{use lower case for non-random stuff}
We have ${\rm OPT}({\cal I}) = \max_{s \in [0,T]} R(s;{\cal I})$, 
and for any $s \in [0,T]$,
    \[
    R(s;{\cal I}) = n_1v_1q(s) + n_1 v_2 (1-q(s))q(T-s) + n_2 v_2 q(T-s).
    \] %\approx \lambda t$.
\end{proposition}

\proof
    The first statement follows from the definition of ${\rm OPT}({\cal I})$ and the fact that the optimal non-adaptive policy can be taken in the class of policies defined by pairs $(s,T-s)$ in which we  use price  $v_1$ for time $s \in [0,T]$ and price $v_2$ for time $T-s$.  The expression for $R(s; {\cal I})$ follows by considering the expected revenue from a customer with each valuation type then using linearity of expectation.
% \hfill\Halmos 
\endproof

\fi



\iffalse
To analyze the regret of our proposed policy, we first need to decompose the regret into individual terms that are tractable to analyze.  
Let $\widehat s(D)$ be the random amount of time we remain at price $v_1$ after the exploration phase, i.e., $\widehat s(D) = \arg \max_{s \in [0,T-s]} R(s; \widehat {\cal I})$.  
Additionally, we define two ``intermediate'' instances $\cI'$ and $\cI''$, that we make use of in the analysis.  
We define $\cI' := (T-s, n-D, \{ n_1 - D, n_2\}, \{v_1, v_2\}, \lambda)$ to be the remaining instance after the exploration period.  
Note that this instance is random since it depends on the random demand $D$ observed in the exploration period.  
We also define $\cI'' := (T -s, n, \{n_1, n_2\}, \{v_1, v_2\}, \lambda)$, which is almost identical to the original instance except that the time horizon is shortened to $T-s$.  
The following lemma decomposes the regret of our policy in terms of the quantities defined above.

\tl{TODO: Define function $R(\cdot, \cI)$ in a simple way}

\fi

To proceed with the analysis,  we decompose the regret into two parts that we bound separately.
In addition to $\widehat \cI$ as defined above, define $\cI' = (\lambda, {\cal P}, (n_1 - D_1, n_2))$ as the instance which remains after observing the demand $D_1$.
We decompose the regret as follows.

\begin{lemma}[Regret Decomposition]\label{lem:regret_decomp_two_price}
Define $\eta_1 = |\E[{\rm Rev}(\widehat \pi, \cI')] - \E[\opt(\widehat \cI)]|$ and $\eta_2 = |\E[\opt(\widehat \cI)] - \opt(\cI)|$.
Then, ${\rm Regret}(\pi^{\rm LTE}) \leq \eta_1 + \eta_2.$    %\item (Interesting Name 1) $\eta_1 := |\E[ R(\widehat s; {\cal I}')] - \E[R(\widehat s, \widehat \cI)]|$
    %\item (Optimization) $\eta_1 := |\E[R(\widehat s; \cI')] - \E[\opt(\widehat \cI)]|$
    %\item (Interesting Name 2) $\eta_2 := | \E[R(\widehat s, \widehat \cI)] - \E[\opt(\widehat \cI)]|$
    %\item (Estimation) $\eta_2 := |\E[\opt(\widehat \cI)] - \opt(\cI'')|$
    %\item (Interesting Name 3) $\eta_3 := |{\rm OPT}({\cal I}) -  \E[\opt(\widehat \cI)]|$
    %\item (Exploration) $\eta_3 := |\opt(\cI'') - \opt(\cI)| $
\end{lemma}

The above follows \strfwd ly by observing that $\E[{\rm Rev}(\widehat \pi, \cI')]$ is a lower bound on the revenue of our policy since it only accounts for the revenue in the {\em earning} phase. 
% \proof{Proof:} 
% Let ${\cal I}' = (T-s, n-D, \{ n_1 - D, n_2\}, \{v_1, v_2\}, \lambda)$ be the residual instance which results after the exploration period of length $s$.  By definition, our policy $\pi^{\rm LTE}$ achieves expected revenue at least ${\mathbb E}[R(\widehat s ; {\cal I}') ]$, where the expectation is over the random residual instance ${\cal I}'$ and the random policy $\widehat s$ we computed based on what was observed from the exploration phase.  We bound the regret as follows:
% \[
% \begin{split}
%     &\regret(\pi^{\rm LTE}, \cI)  \\
%     &=  {\rm OPT}({\cal I}) - {\rm Rev}(\pi^{\rm LTE}, {\cal I}) \\
%      & \leq {\rm OPT}({\cal I}) - \E[ R(\widehat s; {\cal I}')] \\
%      & \le \left|{\rm OPT}({\cal I}) - \E[\opt(\widehat \cI)]\right| + \left|\E[\opt(\widehat \cI)] -  \E[R(\widehat s, \widehat \cI)]\right| \\
%      &+ \left|\E[ R(\widehat s; {\cal I}')]  - \E[R(\widehat s, \widehat \cI)]\right| \\
%      & =\eta_3 +  \eta_2 + \eta_1.\\
% \end{split}
% \]

% The first inequality follows from the observation above and the last inequality follows from the definitions of $\eta_1,\eta_2,\eta_3$ and rearranging the previous line.
% % \hfill\Halmos 
% \endproof

We will show that 
% analyze each of the error terms defined above to derive a regret bound in terms of the length of the exploration period $s$.   Optimizing 
for suitable $s$, both terms above are $\tilde O(n^{2/3})$.  
%We first show that $\eta_1 =0$.  This will follow because we use unbiased estimates and the error is linear in $\widehat n_i - n_i$.
%This is essential because the error is linear in $\widehat n_i - n_i$, and we are using an unbiased estimator.
To this end, we first show that $\eta_1$ will grow linearly in $s$.  
We need two observations.  First, our estimates are unbiased and the revenue function is linear in $n_j$'s. 
Second, we observe that the impact of the exploration phase is linear in the length $s$ of the exploration phase.

\begin{lemma}[Bounding $\eta_1$] \label{lem:eta1_bound}
%For our policy $\pi^{\rm LTE}$, 
We have $\eta_1 = O(\lambda n p_1 s)$.
\end{lemma}
\iffalse
\proof
First we write $\E[R(\widehat s; \cI')] - \E[\opt(\widehat \cI)]$ as 
$(\E[R(\widehat s; \cI')] - \E[R(\widehat s; \widehat \cI)]) + (\E[R(\widehat s; \widehat \cI)] - \E[\opt(\widehat \cI)])$ and we will show that each of these terms is 0.  
For the first term, we condition on $\widehat s = s$ and consider the conditional expectation  $\E[R(\widehat s; \cI') - R(\widehat s; \widehat \cI) \mid \widehat s = s]$.  For all $s \in [0,T]$, we have
\[
\begin{split}
  R(s; \cI') -& R(s; \widehat \cI) = (n_1 - D - (\widehat n_1 - D))v_1 q(s)  \\
   + & (n_1 - D - (\widehat n_1 - D))v_2 (1-q(s))q(T-s) \\
   +& (n_2 - \widehat n_2)v_2 q(T-s)  
\end{split}
\]
Thus the conditional expectation above is 0.  Applying the law of total expectation implies the first term is 0.  For the second term, this immediately follows from the definition of $\widehat s$ since it witnesses an optimal non-adaptive policy for the instance $\widehat \cI$.
\endproof
\fi  


% \proof{Proof:} We will show that $\E[ R(\widehat s; {\cal I}') - R(\widehat s, \widehat \cI) \mid \widehat s = s] =0$.  The lemma then follows from the law of total expectation.  The only way the instances $\widehat \cI$ and $\cI'$ differ is in the number of type 1 and type 2 customers.  Using this we observe that for any fixed $s \in [0,T]$, we have
% \[
% \begin{split}
%     R(s; {\cal I}') -  R(s, \widehat \cI)  = &  (n_1 - D - (\widehat n_1 - D))v_1 q(s) \\
%       & + (n_1 - D - (\widehat n_1 - D))v_2 (1-q(s))q(T-s) + (n_2 - \widehat n_2)v_2 q(T-s) \\
%       = & (n_1 - \widehat n_1)(v_1q(s) + v_2(1-q(s))q(T-s)) + (n_2-\widehat n_2)v_2q(T-s)
% \end{split}
% \]
% Therefore taking the expectation conditional on $\widehat s = s$, we have
% \[\E[ R(\widehat s; {\cal I}') - R(\widehat s, \widehat \cI) \mid \widehat s = s] = 0\]
% since $\widehat n_1$ and $\widehat n_2$ are unbiased estimates of $n_1$ and $n_2$.
% % \hfill\Halmos 
% \endproof

%The proof of Lemma~\ref{lem:eta1_bound} can be found in the appendix. 
To bound $\eta_2$, we use concentration inequalities to show that our estimates are close to the target values with high probability. 
Specifically, we apply Bernstein's inequality to $D_1 \sim {\rm Binomial}(n_1, q(s))$, and combine this with the approximation $q(s) = 1-\exp(-\lambda s) \approx \lambda s$ for small $\lambda s$.
%Under this condition we can show that the optimal revenue on $\widehat \cI$ is close to the optimal revenue on $\cI$.  
% First we state the lemma and then develop some tools to prove it.

\begin{lemma}[Bounding $\eta_2$] \label{lem:eta2_bound}
We have $\eta_2 = O\lb(p_1\sqrt{\frac {n \log n}{\lambda s}}\rb)$.
\end{lemma}

\iffalse
% Theorem: Hoeffding
The following is a standard concentration inequality for binomial random variables, see, e.g., Theorem 2.26 in~\citealt{VershyninHDP}.
We will use this to show that the estimates $\widehat n_i$ we compute in the learning phase are likely to be close to the true values $n_i$.

\begin{theorem}[Concentration, Binomial Distribution] \label{thm:concentration}
Let $X \sim {\rm Binomial}(n,p)$, then
\[
\Pr[|X- \E[X]| > \epsilon] \leq 2\exp(-2\epsilon^2/n).
\]
\end{theorem}


\begin{definition}[Clean Event]
Define ${\cal E}$ to be the event that for all $i\in \{1,2\}$, $|\widehat n_i - n_i| \leq \sqrt{4 n \log(n)} / \lambda s$.  We call this the \emph{clean event}.  
\end{definition}


% Lemma: Clean event
\begin{lemma}[Clean Event is Likely]\label{lem:clean_event}
    We have $\\Pr[{\cal E}] \geq 1- 2n^{-2}$ whenever $\lambda s\leq 1.59$.
\end{lemma}
\fi
% Proof sketch: apply the previous theorem and the definition of the estimates $\widehat n_i$
\iffalse
\proof
Since $n_2 = n - n_1$ and $\widehat n_2 = n - \widehat n_1$, it suffices to show $|\widehat n_1 - n_1| \leq \sqrt{4 n \log(n)} / \lambda s$ with probability $1-2n^{-2}$.  Recall that $\widehat n_1 = D/q(s)$, where $D \sim {\rm Binomial}(n_1, q(s))$.  Applying Theorem~\ref{thm:concentration} to $D$, we have
\[
    \Pr[|D - n_1q(s)| > \sqrt{n \log(n)}] \leq \frac{2}{n^2}
\]
Applying this to $\widehat n_1$, we have that
\[
|\widehat n_1 - n_1| = \frac{|D - n_1q(s)|}{1-\exp(-\lambda s)} \leq \frac{\sqrt{4 n \log(n)}}{ \lambda s}
\]
with probability $1-\frac{2}{n^2}$, as claimed.  Here we used the inequality $\exp(-\lambda s) \leq 1-\lambda s/2$ for $\lambda s \leq 1.59$.
\endproof
\fi


\iffalse
% f-g lemma
\tdtl{Let's move the purple part to apdx? This would make the structure better.}
{\color{purple} The following lemma states that if two functions are point-wise close, then their maximums are also close.  
This essentially follows from the triangle inequality.

\begin{lemma}[$3\epsilon$-\ineq]\label{lem:fg_lemma}
Let $f,g$ be real-valued functions defined on any set $\cX$. If for all $x \in \cX$, we have $|f(x) - g(x)| \leq \epsilon$, then $|\max_x f(x) -\max_x g(x)| \leq 3 \epsilon$.
\end{lemma}
}
\fi
% Proof sketch: this is an application of the triangle inequality
\iffalse
\proof 
Let $x^*_f \in \arg\max_x f(x)$ and $x^*_g \in \arg\max_x g(x)$.  By symmetry, it suffices to show $f(x^*_f) - g(x^*_g) \leq 3 \epsilon$.  Expanding this difference, we have
\[\begin{split}
    f(x^*_f) - g(x^*_g)  &=  f(x^*_f) - g(x^*_f) + g(x^*_f) \\
     &-f(x^*_g) + f(x^*_g) - g(x^*_g) \\
     & \leq 2\epsilon + g(x^*_f) - f(x^*_g) \leq 3 \epsilon.
\end{split}\]
The first inequality follows from the condition on $f$ and $g$, and the second inequality follows since $g(x^*_f) - f(x^*_g) \leq g(x^*_g) - f(x^*_g) \leq \epsilon$.
\endproof
\fi
\iffalse
Lemma \ref{lem:eta2_bound} then follows by
% we consider bounding $\eta_2$ under both the clean event ${\cal E}$ and its negation.  For the clean event, 
% we use Lemma~\ref{lem:fg_lemma} along with the error bound implied by ${\cal E}$ with  
choosing the functions $f = {\rm Rev}(\cdot, \widehat \cI)$ and $g = {\rm Rev}(\cdot, \cI)$, and choose $\eps$ to be  the bound implied by Bernstein's \ineq.
% For the other case, we have that $\Pr[\neg {\cal E}] \leq 2n^{-2}$ so the expected contribution is $o(1)$.
\fi

% Proof eta_2 lemma
\iffalse
\proof[Proof of Lemma~\ref{lem:eta2_bound}]
We want to bound $|\E[\opt(\widehat \cI)] - \opt(\cI)]|$.  
We do this under two conditions ${\neg \cal E}$ and ${\cal E}$, where ${\cal E}$ is the event defined in Lemma~\ref{lem:clean_event}.
For the first case, this difference is at most $nv_1$ and $\Pr[\neg {\cal E}] \leq 2n^{-2}$, so the expected contribution for this case is $o(1)$.  For the second case, observe that for any $D, \widehat n_1, \widehat n_2$, and any policy $\pi$, we have
\[
|{\rm Rev}(\pi, \widehat \cI) - {\rm Rev}(\pi, \cI)| \leq |\widehat n_1 - n_1|v_1 + |\widehat n_2 - n_2| v_2
\]
Under event ${\cal E}$, we have $|\widehat n_i - n_i| \leq O(\sqrt{n \log (n)}/\lambda s)$. 
Since this holds for all feasible policies $\pi$, we may apply Lemma~\ref{lem:fg_lemma} with $f = {\rm Rev}(\cdot, \widehat \cI)$ and $g = {\rm Rev}(\cdot, \cI)$ and taking $\epsilon$ to be the bound above to get a bound on $\eta_2$ under event ${\cal E}$.
Combining the bounds under each event yields the lemma.
\endproof
\fi

\iffalse
\su{My simplistic view: cond on the clean event. Then, observe that for any realization of D and $D' = \widehat n_1 - n_1$, the difference is $O(D+D')$. Done by taking expectation.}
We want to bound $|\E[\opt(\widehat \cI)] - \opt(\cI'')]|$.  
We do this under two conditions ${\cal E}$ and $\neg {\cal E}$, where ${\cal E}$ is the event defined in Lemma~\ref{lem:clean_event}.  
For the second case, this difference is at most $nv_1$ and $\Pr[\neg {\cal E}] \leq 2/n^2$, so the expected contribution to $\eta_2$ for this case is $o(1)$.
For the second case, we observe that for fixed $\widehat \cI$ (in general this instance is random since it depends on $D$) and for $\cI''$, that $\opt(\widehat \cI) = \max_{s'} R(s'; \widehat \cI)$ and $\opt(\widehat \cI'') = \max_{s'} R(s'; \widehat \cI'')$.  Under the event ${\cal E}$, we have that
\[
|R(s; \widehat \cI) - R(s; \cI'')| \leq 2 v_1 \epsilon
\]
for all $s \in [0,T-s]$ and $\epsilon$ as defined in Lemma~\ref{lem:clean_event}.  So applying Lemma~\ref{lem:fg_lemma}, with $f = R(\cdot ; \widehat \cI)$ and $g = R(\cdot; \cI'')$ completes the proof.
\fi

\iffalse
% eta_3 bound
\begin{lemma}[Analysis of $\eta_3$] \label{lem:eta3_bound}
$\eta_3 \leq \frac{s}{T} \opt(\cI)$.
\end{lemma}

Before proving this, we recall the following simple inequalities.

\begin{proposition}[Inequality for $\exp(\cdot)$] \label{prop:exp_inequalities}
    For all $x \in \mathbb{R}$ and $\alpha \in (0,1)$ we have
    \[1- \exp(-\alpha x) \geq \alpha(1-\exp(-x)).\]
\end{proposition}
\proof
Since $e^{x}$ is convex, we can write $-\alpha x$ as the convex combination $\alpha(-x) + (1-\alpha)0$.  Thus, 
\[
\exp(-\alpha x) \leq \alpha \exp(-x) + (1-\alpha) \exp(0).
\]
Simplifying and rearranging yields the claim.
\endproof


% Proof sketch: scale the optimal non-adaptive policy down to the time horizon $T-s$.
\proof 
Since the only difference between $\cI$ and $\cI''$ is that the latter has a shorter time horizon of $T-s$ it suffices to upper bound $\opt(\cI) - \opt(\cI'') \geq 0$.  
In particular, the claim follows if $\opt(\cI'') \geq \frac{T-s}{T} \opt(\cI).  $ Let $s^* = \arg \max_{s' \in [0,T]} R(s'; \cI)$ witness the optimal non-adaptive policy for the two price case.  We get a policy for instance $\cI''$ by taking $s'' = s^* (T-s)/T$ and observe that this gives us a lower bound on $\opt(\cI'')$.  Thus
\[
\begin{split}
\opt(\cI'') \geq & R(s''; \cI'') \\ 
= & n_1v_1(1-\exp(-\lambda s'')) \\ 
+ & n_1v_2 \exp(-\lambda s'') (1-\exp(-\lambda (T-s-s''))) \\ 
+&  n_2v_2(1-\exp(-\lambda (T-s-s'')))
\end{split}
\]
Note that $\exp(-\lambda s'') \geq \exp(-\lambda s^*)$ since $s'' \leq s^*$. 
The other terms we bound by using Proposition~\ref{prop:exp_inequalities} with $\alpha = \frac{T-s}{T} \in (0,1)$ and $x= s^*$, then again with the same $\alpha$ and $x = T-s^*$ to conclude that $R(s''; \cI'') \geq \frac{T-s}{s} R(s^*; \cI) = \frac{T-s}{T}\opt(\cI)$.
\endproof
\fi

\iffalse
\proof[Proof of Theorem~\ref{thm:regret_bound} (Two Price Case)]
Using Lemmas~\ref{lem:regret_decomp_two_price}, ~\ref{lem:eta1_bound}, ~\ref{lem:eta2_bound}, ~\ref{lem:eta3_bound} we can bound the regret as follows:
\[
\begin{split}
  {\rm Regret(\pi^{\rm LTE})} \leq & O(v_1\sqrt{n_1 \log(n)} / \lambda s + v_1 \sqrt{n_1 \log(n)}) \\
   &+ \frac{s}{T}\opt(\cI)+  o(1) .
\end{split}
\]
With the further bound that $\opt(\cI) \leq \lambda n v_1 T$ and taking $s = \Theta(n^{-1/4} / \lambda)$, we get the claimed bound on the regret.
\endproof
\fi

Completing the analysis for the two-price case, 
from Lemmas~\ref{lem:regret_decomp_two_price}, ~\ref{lem:eta1_bound}, and~\ref{lem:eta2_bound} we have
\[{\rm Regret}(\pi^{\rm LTE}) \leq O\left(\lambda n p_1 s +  p_1 \sqrt{\frac {n \log (n)}{\lambda s}}\right).
\]
The $\tilde O(n^{2/3})$ bound follows by taking $s=  n^{-1/3} / \lambda$.

\subsection{Extending to \texorpdfstring{$k$}{K} Price Levels}
The analysis for the $k$-price setting is more involved since we need to carefully analyze how the estimation errors accumulate. 
In particular, rather than bounding the estimation errors $\widehat n_j - n_j$ individually, we prove a novel concentration inequality for the total estimation error $\sum_{j \in [k]}(\widehat n_j - n_j)$.  
{\new The first challenge is dependence: $\widehat n_j$ depends on each $\widehat n_i$ for $i \leq j-1$.}
% This does not easily follow from standard concentration bounds such as Hoeffding's inequality or Bernstein's inequality since we do not have independence; .  
Additionally, we will see that the process $Y_j = \sum_{i \leq j} (\widehat n_i - n_i)$ does not form a martingale, so Azuma's inequality does not apply either. 
We address this by showing that the process admits a {\em self-neutralizing} property that allows us to apply the Cram{\'e}r-Chernoff method to get a concentration bound.

\subsubsection{Decomposition of Regret}

To set up the analysis, recall that $\eta_1 + \eta_2$ is an upper bound on the regret of our policy, where $\eta_1 = |\E[{\rm Rev}(\widehat \pi, \cI')] - \E[\opt(\widehat \cI)]|$ and $\eta_2 = |\E[\opt(\widehat \cI)] - \opt(\cI)|$.  
We define $ \widehat {\cal I}$ as in Algorithm~\ref{alg:learn_then_earn}, but now we define ${\cal I}' = {\rm UDPM}(\lambda, {\cal P}, (N_j)_{j \in [k]})$, where $N_j$ is the random number of type-$j$ customers remaining after the learning phase.  
First, we generalize \cref{lem:eta1_bound} to the $k$-price setting.

\begin{lemma}[Bounding $\eta_1$ in $k$-price setting] \label{lem:k_price_eta1_bound}
It holds that $\eta_1 = O(\lambda n p_1 \sum_{j=1}^k s_j)$.
\end{lemma}

% This again essentially follows since we use unbiased estimates and the revenue is linear in the size of each price segment. We also use the fact that the impact of the exploration phase is linear in $\sum_{j=1}^k s_j$.

The main challenge is in bounding $\eta_2$, where we need to ensure that estimation errors accumulate slowly.  
Recall that $\eta_2 = |\E[\opt(\widehat \cI)] - \opt(\cI)| = |\E[ \max_{x} {\rm Rev}(x, \widehat \cI) -  \max_x {\rm Rev}(x, \cI)|$. 
%Using  \cref{lem:fg_lemma} and some standard bounds, we obtain the following.
Using some standard bounds, we obtain the following.

\begin{lemma}[Bounding $\eta_2$ in the $k$-price setting] \label{lem:k_price_eta2_bound}
For all $t > 0$, we have
\[\eta_2 \leq  3 \cdot \left(t + p_1n \Pr[ \sup_{x} |R(x, \widehat \cI) - R(x, \cI)| > t] \right).\]
\end{lemma}


\subsubsection{Bounding the Revenue Deviation}
With \cref{lem:k_price_eta2_bound}, we want to show $\sup_{x} \lb|R(x, \widehat \cI) - R(x, \cI)\rb|$ can not be too large, formalized below.

\bprop[Deviation of Revenues]\label{prop:dev_rev}
For any $t>0$, we have \[\Pr\lb[\sup_{x} \lb|R(x, \widehat \cI) - R(x, \cI)\rb| >t\rb] \leq 2(k+1)\exp \lb(-t^2/(p_1^2n \sum_{j=1}^k (1/q(s_j)) \rb).\]
\eprop

Taking $t = \tilde \Theta( p_1 \sqrt{n \sum_{j=1}^k \frac{1}{q(s_j)}})$ and combining with  Lemma~\ref{lem:k_price_eta2_bound}, we obtain the following.

\bcoro[Bounding $\eta_2$] It holds that  $\eta_2 \leq \tilde{O}(p_1 \sqrt{n \sum_{j=1}^k \frac{1}{q(s_j)}})$
\ecoro
  
The key step to prove \cref{prop:dev_rev} is to show that  $R(x, \widehat \cI) - R(x, \cI)$ is $\sigma$-subgaussian  for any fixed non-adaptive policy $x$, where $\sigma^2 = O(p_1^2 n \sum_{j=1}^k \frac{1}{q(s_j)})$.
% for any fixed non-adaptive policy $x$, 
To this end, for any fixed any instance $\cI$, we write
${\rm Rev}(x, \cI) = \sum_{j=1}^k R_j(x) n_j$, where $R_j(x)$ is the expected revenue of a customer with valuation $p_j$ under the non-adaptive policy $x$.  
Then, \[{\rm Rev}(x, \widehat \cI) - {\rm Rev}(x, \cI) = \sum_{j=1}^k R_j(x)(\widehat n_j - n_j).\]
Note that for any fixed non-adaptive policy $x$, we have $p_1 \geq R_1(x) \geq R_2(x) \geq \ldots \geq R_k(x) \geq 0$.  

% definitions and theorem statement

Thus, non-adaptive policies map to non-increasing non-negative sequences of weights on the customer segment sizes $(n_j)_{j \in [k]}$.  
Due to this mapping, we will argue about such sequences directly.  
Given $r \in [0, p_1]^k$ representing such a sequence we let $Y_j(r) = \sum_{i \leq j} r_i (\widehat n_j - n_j)$.  
Our goal is to show that $Y_k(r)$ is sub-gaussian for each such $r$.  

\subsubsection{Self-Neutralizing Process and Conditional Subgaussianity}
To accomplish this, we identify two properties that allow us to apply the Cram{\'e}r-Chernoff method to $Y_k(r)$ to show sub-gaussianity.  
In the following two definitions, let  $(\Delta_j)_{j \in [k]}$ be a sequence of mean zero random variables adapted to the filtration $({\cal F}_j)_{j \in [k]}$.
In our context, we will take $\Delta_j = \widehat n_j - n_j$.
The first definition establishes what we call a self-neutralizing process and the second states that each term in the process is sub-gaussian when conditioned on the past.

\begin{definition}[Self-Neutralizing Process] \label{def:self_neutralizing_process}
We say $(\Delta_j)_{j \in [k]}$ is a {\em self-neutralizing} process if for all $j \in [k]$, we have
$\E[\Delta_j \mid {\cal F}_{j-1}] = - \sum_{i \leq j-1} \Delta_i.$
\end{definition}

\begin{definition}[Conditionally Sub-gaussian] \label{def:conditional_subgaussian}
We say $(\Delta_j)_{j \in [k]}$ is conditionally sub-gaussian if there exists $(c_j)_{j \in [k]}$ such that for all $j \in [k]$ and $\gamma > 0$, we have
\[
\E[ \exp(\gamma \Delta_j) \mid {\cal F}_{j-1}] \leq \exp \left( \gamma \E[\Delta_j \mid {\cal F}_{j-1}] + \gamma^2 c_j^2/2 \right).
\]
\end{definition}


Taken together, these imply the following theorem, which may be of independent interest.

\begin{theorem}[MGF Bound] \label{thm:mgf_bound}
Let $(\Delta_j)_{j \in [k]}$ be a self-neutralizing process and conditionally sub-gaussian with constants $(c_j)_{j \in [k]}$.  For any non-increasing, non-negative sequences of constants $(r_j)_{j \in [k]}$, denote $Y_k(r) = \sum_{j \leq k} r_j \Delta_j$. Then, for  all $\gamma > 0$, we have
\[
\E[\exp(\gamma Y_k(r))] \leq \exp\left(\gamma^2 \sum_{j = 1}^k (r_j c_j)^2 /2 \right).
\]
\end{theorem}


The overall strategy is similar to the proof of the Azuma-Hoeffding inequality, but due to the impact of the weight sequence $(r_j)$, we need to be  careful with how we apply induction.
% The proof is deferred to the Appendix.  

\subsubsection{Proof Outline of \cref{prop:dev_rev}}
Taking $\Delta_j = \widehat n_j - n_j$ and ${\cal F}_j = \sigma(D_1, D_2,\ldots, D_j)$, it can be shown that this sequence satisfies Definitions~\ref{def:self_neutralizing_process} and~\ref{def:conditional_subgaussian} with $c_j^2 = 2\sum_{i \leq j} n_i / q(s_j)$.  
Both proofs have been deferred to the Appendix, but we remark that the first follows straightforwardly from the definition of our estimator.  
The second relies on the fact that $D_j\sim {\rm Binomial}(\sum_{i \leq j} n_i - \sum_{i \leq j-1} D_i, q(s_j))$.  
As a consequence of the Cram{\'e}r-Chernoff method, we can apply Theorem~\ref{thm:mgf_bound} to $\Delta_j = \widehat n_j - n_j$ to get that for all non-increasing, non-negative sequences $r$:
\[
\Pr\lb[ \lb|\sum_{j=1}^k r_j(\widehat n_j - n_j) \rb| > t \rb] \leq 2 \exp\lb( -\frac{t^2}{4 \sum_{j=1}^k r_j^2\sum_{i\leq j} n_i / q(s_j)} \rb) \leq 2 \exp\lb( -\frac{t^2}{4 r_1^2n \sum_{j=1}^k (1/ q(s_j))} \rb).
\]
The second inequality uses that $r_j \leq r_1$ and that $\sum_{i \leq j} n_i \leq \sum_i n_i = n$.
Thus, by taking $r_j = R_j(x)$ for some $x$ we get the same bound on $|{\rm Rev}(x, \widehat \cI) - {\rm Rev}(x, \cI)|$ for any non-adaptive policy $x$.

Next, we need to apply a union bound argument to upgrade the above bound to a bound on $\sup_x|{\rm Rev}(x, \widehat \cI) - {\rm Rev}(x, \cI)|$.  
There are infinitely many such non-adaptive policies making, a na\"{i}ve union bound vacuous.  
In this case, a standard approach is to union bound over an $\epsilon$-cover of the set of non-adaptive policies, but these can grow super-polynomially in $k$.  
Instead, we will use the connection to non-increasing, non-negative weight sequences in $[0,p_1]^k$ and show that it suffices to union bound over only $k+1$ such sequences.  
This is formalized in the following lemma.

\begin{lemma}[Convex Combination] \label{lem:convex_comb_argument}
    For $j\in \{0\} \cup [k]$, let $e_j \in \ho{R}^k$ be the vector with the first $j$ entries set to 1 and the last $k-j$ entries set to 0.  We have the following:
    \begin{itemize}
        \item If $|Y_k(r)| \leq t$ and $|Y_k(r')| \leq t$, then for all $ \alpha \in [0,1]$, $|Y_k(\alpha r + (1-\alpha) r')| \leq t$
        \item Any non-increasing sequence $r \in [0,1]^k$ is a convex combination of $\{e_j\}_{j=0}^k$
    \end{itemize}
\end{lemma}

The proof of this lemma is straightforward since $Y_k(r)$ is linear in $r$.
% see the appendix.
This implies that we only need to union bound over the set $\{e_j\}_{j=0}^k$ of size $k+1$.  As a consequence, we obtain
\begin{equation} \label{eqn:sup_error_tail_bound}
    \Pr\lb[ \sup_x|{\rm Rev}(x, \widehat \cI) - {\rm Rev}(x, \cI)| >t \rb] \leq 2(k+1) \exp\lb( -\frac{t^2}{4 r_1^2n \sum_{j=1}^k (1/ q(s_j))} \rb),
\end{equation}
and \cref{prop:dev_rev} follows.

\subsubsection{Concluding the Proof}
Now to complete the analysis.
Take $s_j = s$ for all $j \in [k]$.
By \cref{lem:k_price_eta1_bound}, we have $\eta_1 = O(\lambda p_1 k n s)$.
Next we combine \eqref{eqn:sup_error_tail_bound} with Lemma~\ref{lem:k_price_eta2_bound}, taking $t= p_1\sqrt{8 kn \log(nk) /q(s)}$ to get $\eta_2 = \tilde{O}(p_1\sqrt{kn / (\lambda s)})$ for small enough $\lambda s$.  Combining these, we have
\[
{\rm Regret}(\pi^{\rm LTE}) = \tilde{O}\lb( \lambda p_1 k n s + p_1\sqrt{ \frac{kn}{\lambda s}} \rb).
\]
By taking $s = \tilde\Theta(\lambda^{-1} (kn)^{-1/3})$ we get a final bound of $\tilde{O}\lb( p_1 (kn)^{2/3}\rb)$.








\iffalse


% Not necessarily old, we just have newer ideas now
We decompose the demand in any phase $j$ as 
\[D_j= D_j^{(1)}+\cdots + D_j^{(j)}\]
where $D_j^{(i)}$ denotes the demand in phase $j$ from customers with valuation $p_i$.
As in the previous section,  we define $\mathcal{I}' = {\rm UDPM}(\lam, \mathcal{P},\{n'_j\})$ where $n_i' =n_i- \sum_{j=i}^k D_j^{(i)}$ for each $i\in [k]$, and $\widehat{\mathcal{I}} = {\rm UDPM}(\lam, \mathcal{P},\{\widehat n_j\})$.
The analysis involves separately bounding \[\eta_1:= \lb|\ho{E}\lb[{\rm OPT}(\widehat{\cal I})\rb] - \ho{E} \lb[{\rm Rev}\lb(\widehat \pi, {\cal I}'\rb)\rb]\rb| \quad\text{and}\quad \eta_2:= \lb|{\rm OPT}(\cal I) - \ho{E}\lb[{\rm OPT}(\widehat{\cal I})\rb]\rb|.\]

The easier part is bounding $\eta_1$.
As in the two-price setting (Lemma \ref{lem:eta1_bound}), it is \strfwd\ to bound $\eta_1$ linearly in the length of the exploration phase, i.e.,
$\eta_1 = O\lb(\lam n \sum_{i=1}^k s_i\rb).$ 

The challging part is bounding $\eta_2$. To obtain a regret sublinear in $k$, we need $\eta_2$ to scale sublinear in $k$. 
To this end, we rewrite the estimator in \eqref{eqn:estimates} as follows.
Recall that for each $j\in [k]$, we have
\[D_j= D_j^{(1)}+\cdots + D_j^{(j)}\]
where $D_j^{(i)}$ denotes the demand from valuation group $i$ in phase $j$.
Unfortunately, instead of observing each individual $D_j^{(i)}$, we can only observe their {\bf sum} $D_j$. 
However, we can estimate them using \[\widehat D_j^{(i)} = (1-q_1-\cdots-q_{j-i})\cdot  \widehat n_i q_j, \quad i\le j-1.\]
Noting that $n_j = D_j - D_j^1 - \dots - D_j^{j-1}$, 
so we use  
\[\widehat n_j := \frac{D_j - \widehat D_j^{(1)} - \cdots - \widehat D_j^{(i-1)}}{q_j}\]
to estimate the number of customers with valuation $p_j$.
It is \strfwd\ to verify that this is equivalent to the estimator given by Eq. \eqref{eqn:estimates}.
Then,
\begin{align}\label{eqn:122923b}
|\widehat n_j - n_j| &= \lb|\frac{D_j - \widehat D_j^1 - \cdots - \widehat D_j^{i-1}}{q_j} - n_j\rb|\notag\\
&\le \lb|\frac {D_j}{q_j} - n_j\rb| +  \frac 1{q_j} \lb|\sum_{i=1}^{j-1} \lb(D_j^{(i)} - \widehat D_j^{(i)}\rb)\rb|\notag \\
&\le \sqrt{\frac {n_j \log n}{q_j}} + \frac 1{q_j} \sqrt{q_j n\log n} \notag\\
&\le 2\sqrt {\frac{n\log n}{q_j}},
\end{align}
where the second \ineq\ is by Bernstein's \ineq.
% Note that $\sum_{i=1}^j n_i\le n$, so \[\eqref{eqn:122923b} \le\sqrt{\frac{\log n}{\lam s_j}}\cdot \sqrt{jn}.\]
Summarizing, we have the following bound on the estimation error.
\begin{lemma}[Bounding the Estimation Error] 
For any $j\in [k]$, we have 
\[|n_j - \widehat n_j| = O\lb(\sqrt {\frac{n\log n}{\lam s_j}}\rb).\]   
\end{lemma}

% We conclude by showing that $\eta_2 = O(\max_{j\in [k]} |n_j - \widehat n_j|)$.
% Recall that from Eq. \eqref{eqn:122523b} that
% the revenue function for any non-\adap\ policy $X$ is ${\rm Rev}(X, \mathcal{I}) =\sum_{\ell=1}^k c_\ell n_\ell$ where  
% \[c_\ell = c_\ell(X,{\cal I}):=\sum_{j:\ell\le j \le k} p_j e^{-\lambda (t_j - t_\ell)} \left(1-e^{-\lambda \lb(t_{j+1} - t_j\rb)}\right)\ge 0.\]
% We show that the revenue function is not only a linear but actually {\em subconvex} combination of $n_i$'s. 

% \begin{lemma}[Sub-\cvx\ combination in $n_j$'s]\label{lem:subcvx}
% For any UDPM \ins\ $\cal I$ and non-\adap\ policy $X$, we have $\sum_{\ell=1}^k c_\ell(X,{\cal I}) \le 1$.
% \end{lemma}

Note that the revenue functions under the true instance $\mathcal{I}$ and the estimated \ins\ $\widehat{\mathcal{I}}$ differ by $\sum_{j\in [k]} |\widehat n_j - n_j|$.
Thus, by Lemma \ref{lem:fg_lemma}, on the clean event we have \[|{\rm OPT}({\widehat {\cal I}}) - {\rm OPT}({\cal I})|= O\lb(k\sqrt {\frac{n\log n}{\lam s}}\rb).\]
Combining, we have 
\[{\rm Reg}(\pi^{\rm LTE}) \le \eta_1 + \eta_2 = O\lb(\lam n ks\rb) + O\lb(k\sqrt {\frac{n\log n}{\lam s}}\rb).\]
We conclude the proof by noticing when $s= n^{-1/3}\lam^{-1}$, the above becomes $\tilde O(k n^{2/3}\log^{1/3} n)$.

\fi


\iffalse 
% OLD 
We briefly sketch how we extend the analysis from two price levels to $k$ price levels.  

Our current analysis for the two-price setting only leads to a bound that depends linearly on $k$.  
% Naive bounds show that the terms $\eta_1$ and $\eta_2$ grow linearly in $k$, leading to an overall bound of $\tilde O(kn^{3/4})$. 
To achieve a sublinear dependence on $k$, we need to be more careful in our analysis of the \emph{total} error in our estimates $\widehat n_i$.  
Due to the dependencies that exist between our estimates $\widehat n_i$, we cannot directly apply concentration inequalities to control the total error.
Instead, we employ a more careful analysis, showing that the sequence $Z_i = \sum_{j \leq i} (\widehat n_j - n_j) - \alpha_i$ is a supermartingale for an appropriate choice of $\alpha_i > 0$.  Then, we apply the Azuma-Hoeffding inequality to obtain a bound that is sublinear in $k$ for the total error.  Using this in the rest of our analysis leads to the $\tilde O(k^{2/3} n^{3/4})$ bound on the regret.  
We defer the details to the appendix.
\fi

\iffalse
We briefly sketch how we extend the analysis from two price levels to $k$ price levels.  
There are two main challenges that arise in this case.
First, when we explore price $v_1$ we may use the same unbiased estimate as in the two price case, but then for prices $v_2, v_3, \ldots, v_{k-1}$ our observed demand contains additional noise that we must adjust for in order to get an unbiased estimate for $n_2, n_3,\ldots, n_{k-1}$.
This is because customers  with higher valuations may purchase during these exploration periods.
We show how to adjust our estimates for this noise to get unbiased estimates.

Second, in order to get regret that is sublinear in $k$ we need to use a more careful analysis of how estimation errors propagate.
A simple generalization of our analysis will instead incur regret that is linear in $k$ since it will allow errors in each estimate to propagate additively.
To address this we show that a small adjustment to the sequence $Y_i = \sum_{j \leq i} (\widehat n_j - n_j)$ forms a supermartingale,
%conditioned on HP event
and thus we may apply Azuma's inequality to get a bound on the total error that is sublinear in $k$.

The remaining parts of our analysis generalize naturally.  
The regret decomposition in Lemma~\ref{lem:regret_decomp_two_price} extends to the $k$ price case where now we now we define the instances $\widehat \cI,  \cI'$, and $\cI''$ to appropriately account for $k$ price levels instead of two.
Moreover, the analysis for $\eta_1$ and $\eta_3$ extend  to this case.  
The main challenge is the analysis of $\eta)_2$ involving supermartingales and Azuma's inequality which we discussed above.
\fi

\iffalse
\[
ksn + \sqrt{nk}/s   --->
\]

Take $s=n^{-1/4}k^{-1/4}$. Regret is $k^{2/3} n^{3/4}$.
\fi













%%%% OLD
\iffalse
In this section we consider discrete demand functions.  Let $v_1 \geq v_2 \geq \ldots \geq v_k$ be a discrete set of $k$ valuation levels and $n_1,n_2,\ldots,n_k$ with $\sum_i n_i = n$ be the number of customers at each valuation level.  Given such a set of valuation levels and number of customers at each level, we let $D(x \mid \{(v_i,n_i)\}_{i=1}^k) = \sum_{i: v_i \geq x} n_i / n$ be the demand function parameterized by the $v_i$'s and the $n_i$'s.  We let $\mathcal{F}_k$ be the class of demand functions parameterized as above by some set of valuation and customer levels.  In our setting, we assume that the decision maker has access to the set of valuation levels $v_1,\ldots,v_k$ and the total market size $n$, but does not know the number $n_i$ of customers at each valuation level $v_i$.

Motivated by the previous section, we consider non-adaptive policies which know the underlying demand function as the class of benchmark policies.  Thus our goal is to find an adaptive policy that has low regret against the optimal non-adaptive policy for any discrete demand curve in the class $\mathcal{F}_k$.  More precisely, we show the following theorem.

\begin{theorem} \label{thm:regret_bound}
    Let $\{(v_i, n_i)\}_{i=1}^k$ be a set of valuations and number of customers at each valuation such that $v_1 \geq v_2 \geq \ldots v_k$ and $\sum_i n_i = n$.  There exists an adaptive policy $\pi^{\rm LTE}$ which satisfies
    \[{\rm Rev}(\pi,\]
\end{theorem}

\fi


%%%%% OLD Version, saved just in case we want to use/modify later

\iffalse

\iffalse
In this section, we \su{state our results in words and give high-level ideas (how the policies work, how the analysis go, ...)}

\subsection{Naive Learn-then-Earn Policy}
Prove our latest results 

\subsection{A Better Policy}
\su{we don't have this yet..}
\fi

Now we consider adaptive policies in the presence of an unknown demand curve.  Our policies attempt to simultaneously learn the demand function and optimize their pricing decisions given a finite time horizon and limited number of price changes.  As is standard in the demand learning literature, we will analyze the \emph{regret} of our policies, which measures the difference in revenue of the proposed policy to the best policy in a class of \emph{benchmark policies}, which are usually equipped with additional information not available to our policy.  As before, we consider the worst case regret against a family of demand functions $\mathcal{F}$.  This leads to the following definition.

\begin{definition}[Worst-Case Regret]
    Let $\mathcal{F}$ be a family of demand functions and $\Pi$ be a class of policies.  The worst case regret of a policy $\pi$ is given by
    \[
    \textrm{Regret}(\mathcal{F}, \Pi, \pi) := \sup_{D \in \mathcal{F}} \sup_{\pi^* \in \Pi} \left(\textrm{Rev}(\pi^*, D) - \textrm{Rev}(\pi, D) \right)
    \]
\end{definition}

% Thomas: do we prefer the term "market size" or "number of customers" to refer to the quantity $n$?
In particular, we are interested in quantifying how the regret of our proposed policies scale with the market size/number of customers $n$.  As $n \to \infty$, our policies revenue should approach that of the best policy in the benchmark class $\Pi$.  

\iffalse
The above definition is general and applies to a wide variety of settings.  Presently, we focus on the following classes of demand functions and pricing policies.  We consider discrete demand functions with support size $k$.  Formally, define $\mathcal{F}_k$ as the following class of functions:

\begin{equation} \label{eqn:k_pt_discrete_demand}
    \mathcal{F}_k := \left\{ F:[0,1] \to [0,1] \mid \exists n_1, n_2,\ldots, n_k \text{ s.t. } \sum_i n_i = n \text{ and } F(x) \sum_ \right\}
\end{equation}

\fi

\subsection{Naive Learn-then-Earn Policy}

To start, we consider the case of the demand function coming from a one parameter linear family and compare against non-adaptive $m$ price change policies which know the underlying demand function as the class of benchmark policies.  Recall that the class of one parameter linear demand functions is given by $\mathcal{F} = \{D(\cdot; \theta):[0,1] \to [0,1] \mid D(x; \theta) = 1-\theta x, \ \theta \in [0,1]\}$.  As discussed before \textcolor{red}{(point a reference back to where we discuss this class of policies)}, this class captures \ldots.  In this case, we show that a simple learn-then-earn policy achieves low regret.  Our goal is to show the following.

\begin{theorem}
    Let $\mathcal{F}$ be the class of one parameter linear demand functions and let $\Pi$ be the class of non-adaptive $m$ price change policies.  There exists a policy $\pi^{{\rm LTE}}$ which achieves $\textrm{Regret}(\mathcal{F}, \Pi, \pi^{{\rm LTE}}) = \tilde{O}(n^{3/4})$.
\end{theorem}

Before diving into the proof, we first describe our policy.  Our policy is parameterized by a pair $(t_1,p_1) \in [0,T] \times [0,1]$ which indicate the length of the initial sales period and the price to set.  These will be chosen in order to minimize the regret.  The steps of the policy $\pi^{\textrm{LTE}}$ is as follows.

\begin{enumerate}
    \item Use price $p_1$ for time $t_1$, observing sales $S_1$.
    \item Construct an estimate $\widehat{\theta}$ based on the observed sales $S_1$.
    \item Compute an optimal sequence of $m-1$ price changes $(p_2,p_3, \ldots, p_m), (t_2,t_3,\ldots,t_m)$ for the remaining time horizon $T-t_1$ and utilize these.
\end{enumerate}

\su{need some work:}

Outline.

Let $N_1$ be the random number of type 1 customers remaining after exploration for time $T'$.  Then we have ${\rm Reg}({\cal A}_{\rm LTO}) \leq A + B + C + D$, where:
\bitem 
\item (Revenue estimation error) $A := |E[R(\widehat s; T-T', N_1, n_2)] -E[R(\widehat s; T-T', \widehat n_1, \widehat n_2)] |$
(idea: concentration)
\item (Optimization error) $B := | E[R(\widehat s; T-T', \widehat n_1, \widehat n_2)] - E[OPT(T-T', \widehat n_1, \widehat n_2)] |$
(idea: = 0 by defn of $\widehat s$)
\item (Optimum estimation error) $C := | E[OPT(T-T', \widehat n_1, \widehat n_2)] - OPT(T-T', n_1, n_2)|$
(idea: use ``f-g'' lemma on the estimation error)
\item (Exploration error) $D := |OPT(T-T', n_1, n_2)] - OPT|$
 (Idea: shrinkage argument)
\eitem 

We next bound A,C,D one by one. Details can be found in our HackMd notes on Jun 29.

\begin{lemma}[Distribution Shift]
Let $\widehat n_1$ and $\widehat n_2$ be the estimators for $n_1$ and $n_2$ given in Claim 1 and $\widehat s$ be the solution computed in our algorithm, then we have:
\[A = |E[R(\widehat s; T-T', N_1, n_2)] -E[R(\widehat s; T-T', \widehat n_1, \widehat n_2)] | \leq E[D_1] v_1 \le n_1 \lambda T' v_1\]
\end{lemma}
Observe that $n_1 = O(n)$, so when $T' = n^{-1/4}$, the above becomes $O(n^{3/4})$. 

\begin{lemma}[Estimation Error on the Optimum]
$C  = | E[OPT(T-T', \widehat n_1, \widehat n_2)] - OPT(T-T', n_1, n_2)| \leq O\left( \frac{\sqrt{n_1 \log (n)}}{ \lambda T'} \right) + o(1)$
\end{lemma}
When $T'=\Theta(n^{-1/4})$, the above becomes $O(n^{3/4})$.

\begin{lemma}[Time Horizon Shrinkage]
$D \le \frac{T'}{T} OPT$. Note that  $T$ is a constant, and $OPT= O(n)$,  so for $T'=n^{-1/4}$, we have $D\le n^{3/4}$.
\end{lemma}

\noindent{\bf Proof of Theorem 2}  Taking $T'= n ^{-1/4}$, we have 
\[Reg \le A+B+C+D \le n^{3/4} + 0 + n^{3/4} + n^{3/4}.\]
% \hfill\Halmos
% \endproof

 \fi

==> OR/Stream.tex <==
Stream + unknown demand: (NEW!) consider valuations $v_1,...,v_k$. 
\benum 
\item Note that under the stream model, we only care about the total amount $(t_i)$  of time at each valuation. 
\Sps\ each buyer has $q_i$ \prb\ of having valuation $v_i$. (note: if $n$ is large, then $q_i \cdot n$ does not differ much from $n_i$)
\item  Then the policy $(t_i)$ has rev is \[n \cdot \sum_i v_i t_i \lb( \sum_{j:j \le i} q_j\rb) = n\cdot \sum_j q_j \sum_{i:i\ge j} v_i t_i, \]
\item Finding the $(t_i)$ for unknown $q_i$: \[\max_{t_i} \min_{q_i} \frac{\sum_i v_i t_i \lb( \sum_{j\ge i} q_j\rb)}{\max_{i} \{v_i \cdot \sum_{j\ge i}q_j\}}\]
\item Thm1. the optimal probability for the stream model is also $t^*$.
\item Show that the pricing policy from the stream model performs worse than the pricing policy for the poo model.

==> OR/nonadap.tex <==

\iffalse 
Our research problem is also related to the robust price optimization problem discussed in \citealt{guan2023randomized}. 
However, they focused on a multi-product scenario where the demand for each product is correlated with the prices of other products. 
They consider the uncertainty of the demand models, while we investigate the uncertainty of the demand distribution.
\fi

{\OKsu
One of the central challenges in pricing is demand uncertainty. 
From now on, we focus on detail-free policies, i.e., those
that do not require knowledge of the demand function $(n_j)_{j\in [k]}$. 
Our objective is to identify policies with robust performance under demand uncertainty.

In this section, we provide a {\em complete} settlement of this problem in the non-adaptive setting.
For any given price set,  we construct a closed-form {\em non-\adap} policy that guarantees a $1/k$ fraction of revenue achievable by any {\bf detail-dependent adaptive} policy.
We also establish minimax optimality: For any non-adaptive, detail-free policy, there is a $k$-price instance on which the revenue is at most $1/k$ times the optimal revenue achievable by any adaptive detail-dependent policy.
{\neww
\subsection{Upper Bound on the Competitive Ratio}
We use the competitive ratio to measure the robustness of a detail-free policy.

\bdefn[Competitive ratio]
Let $\Pi$ be the class of all (possibly adaptive) policies and $\mathcal{F}$ be a family of UDPM instances.
For any $\mathcal{I}\in \mathcal{F}$, define ${\rm OPT}(\mathcal{I})= \sup_{X'\in \Pi} {\rm Rev}(X',\cI)$.
The {\em competitive ratio} of a policy $X$ is
\[{\rm CR}(X, \mathcal{F}) := \inf_{\mathcal{I}\in \cal F} \frac{{\rm Rev}(X, \mathcal{I})}{{\rm OPT}(\mathcal{I})}.\]
\edefn

A policy with a competitive ratio of at least $c$ is called {\em $c$-competitive}.
We note that the competitive ratio is defined for any policy $X$, irrespective of its adaptivity.
Therefore, in the definition of ${\rm OPT}(\mathcal{I})$, it is natural to consider all policies rather than only non-adaptive policies.

We show that no detail-free non-adaptive policy has a competitive ratio better than $1/k$.
\begin{theorem}[Upper Bound on the Competitive Ratio]\label{thm:non_adap_upper} For any $\eps > 0, k \ge 1$ and detail-free non-adaptive policy ${\bf t}$, there is a UDPM instance $\cI_\eps\in \mathcal{F}_k$ such that \[{\rm Rev}({\bf t}, \mathcal{I}_\eps)\le \left(\frac 1k + \eps \right) {\rm OPT}(\mathcal{I}_\eps).\]
\end{theorem}
}
{\neww To prove this, we choose the prices to be a geometric sequence with a common ratio such that $$\frac{1}{k - \sum_{i=1}^{k-1} \frac{p_{i+1}}{p_i}} \le \frac 1k + \frac \eps2.
$$ 
Then, we construct for every $\bf t$ an instance $\cI_\eps$ wherein all customers have the same valuation. 
Furthermore, we choose $\lam$ to be small so that $$\frac{{\rm Rev}(\cI_\eps)}{{\rm OPT}(\cI_\eps)} \le \frac{1}{k - \sum_{i=1}^{k-1} \frac{p_{i+1}}{p_i}} + \frac \eps 2 \le \frac{1}{k} + \eps.$$
We defer the details to Appendix \ref{apdx:UB}.

Here we want to highlight that there exists multiple non-\adap\ policies that can achieve a $1/k$ competitive ratio. 
For example, a naive randomized policy that selects price randomly and commits to it forever guarantees a $1/k$ competitive ratio. 
Similarly, a naive deterministic policy uses the decreasing price sequence each with a time interval $1/k$ will also ensure a $1/k$ competitive ratio. 

\bdefn[Naive  Randomized Policy (NR)]
    A naive randomized policy selects a price uniformly at random and commits to it till the end of the selling season. Formally, a naive randomized policy satisfies
    \begin{align*}
        \Pr(X_s = p_i, s \in [0, 1]) = \frac{1}{k}
    \end{align*}
\edefn

\bdefn[Naive Deterministic Policy (ND)]
    A naive deterministic policy uses the decreasing price sequence each with a time interval $1/k$. Formally, a naive deterministic policy satisfies
    \begin{align*}
        X_s = p_i,  \text{ for } s \in \left[\frac{i-1}{k}, \frac{i}{k}\right).
    \end{align*}
\edefn

\begin{proposition}
    For any UDPM \ins\ $\cal I$ with a $k$-price set, both the naive randomized policy (NR) and the naive deterministic policy (ND) achieve a $1/k$ competitive ratio. 
\end{proposition}
Although both NR and ND achieve a $1/k$ competitive ratio, which aligns with the worst-case bound, neither of them takes the price set into consideration, leading to poor performance in trivial cases. 
For instance, consider a price set $\tilde{\cal P}$ 
comprising $k$ prices evenly spaced between $1$ and $2$.
In this scenario, both NR and ND maintain a competitive ratio of $1/k$, whereas a simple policy that commits to a price of $1$ possesses a competitive ratio of at least $1/2$. 
This example reveals the importance of considering the price set when designing a robust policy.
In the following subsection, we study the max-min optimization for designing the robust pricing policy for any given price set.

% Similarly, the robust stream policy outlined in \cref{sec:robust_stream} also maintains a competitive ratio of $1/k$. However, unlike these straightforward policies, our policy is parametrized by the prices. Notably, the competitive ratio of our policy significantly surpasses that of trivial algorithms in many cases, particularly for continuous price intervals. In the following subsection, we show that for continuous price intervals $[p_{\min}, p_{\max}]$, the competitive ratio of our policy converges to $\frac{1}{1 + \ln (\rho)}$ where $\rho = \frac{p_{\max}}{p_{\min}}$. In contrast, the competitive ratio of the trivial decreasing price sequence converges to 0. This makes our policy substantially different from the trivial algorithms. 
}

\subsection{Max-Min Optimization}

To proceed, we introduce an intuitive upper bound on the revenue of {\bf any} detail-dependent policy.
By Proposition \ref{prop:monotone}, we lose no generality by restricting ourselves to markdown policies.
For any instance $\mathcal{I} = (\lam, \mathcal{P}, (n_j)_{j\in [k]})$ and non-adaptive markdown policy ${\bf t} = (t_j)_{j\in [k]}$, consider  $f({\bf t}; n_1,\dots,n_k):= {\rm Rev}(X, \mathcal{I}) / {\rm OPT}(\mathcal{I}).$
Then, the problem of maximizing the competitive ratio is equivalent to}
{\neww
\begin{align*}
\text{(P0) } & \max_{t_1,\dots,t_k} \min_{n_1, \dots, n_k} \lb\{f(t_1,\dots,t_k; n_1,\dots,n_k): \sum_{j=1}^k n_j=n \rb\},\\
& \text{subject to} \quad \sum_{j=1}^k t_j = 1,
\quad  t_j \ge 0, \quad \forall j \in [k].
\end{align*}
}

{\OKsu 
\subsection{Upper Bound on the Optimum}
Unfortunately, it is challenging to directly solve (P0) - most results on max-min optimization rely on special structures such as concavity-convexity, but $f$ is neither convex in the $n_i$'s nor concave in the $t_i$'s. 
Furthermore, nonconvex-nonconcave min-max optimization is computationally hard \citep{daskalakis2021complexity}. 
% {\new \citep{johnson1988easy,papadimitriou1994complexity,etessami2010complexity,daskalakis2021complexity}.}
% \tdtt{read the lit rev of this paper, and cite earlier papers on the HARDNESS of noncvx-nonconcave min-max opt.}
An alternative idea is to find a closed form formula for the ``min'' part given any $\bf t$, thus reducing (P0) to a single-level problem. 
However, finding a closed-form solution for ${\rm OPT}(\mathcal{I})$ is considerably formidable.
% TL: Cutting next sentence since we redefined OPT.
%In fact, it is quite challenging to even derive a closed-form expression for the revenue of an optimal  {\em non-\adap} policy, given the intricate nature of  the revenue \func\ in \ref{prop:exp_rev}.

We address this challenge from a different perspective.
We first approximate the numerator and denominator of $f$, thus transforming (P0)   into a tractable problem.
Then we argue that this transformation preserves the competitive ratio up to a factor of $k$.
We start by introducing an upper bound on ${\rm OPT}(\mathcal{I})$.
% \bdefn[Upper Bound on the Optimum]\label{def:UB}
% For any UDPM instance $\mathcal{I}=(\lambda, \{p_i\}_{i=1}^k,\{n_i\}_{i=1}^k)$, we define ${\rm UB}(\mathcal{I}):= \sum_{i \in [k]} n_i p_i (1- e^{-\lambda}).$
% \edefn

\begin{proposition}[Upper Bound on the Optimum]\label{prop:ub} 
For any adaptive detail-dependent policy $X$ and instance $\mathcal{I} = {\rm UDPM}(\lambda, \{p_i\}_{i=1}^k,\{n_i\}_{i=1}^k)$, we have
\[{\rm Rev}(X,\mathcal{I}) \le {\rm UB}(\mathcal{I}):= \sum_{i \in [k]} n_i p_i (1- e^{-\lambda}).\]
\end{proposition}

For readers familiar with economics, this upper bound is the revenue achieved by {\em first-degree price discrimination}, modulo a factor of $1-e^{-\lam}$.
To see this \ineq, note that the expected revenue of a customer with a valuation $v$ is at most $v(1-e^{-\lambda})$.
\cref{prop:ub} then follows by summing over all customers.  

Before ending this subsection, we note that this upper bound becomes tighter as $\lam$ increases.
To see this, observe that when $\lam = \infty$, we can achieve (perfect) first-degree price discrimination by moving from the highest price to the lowest price, hence the identity holds.
On the other extreme, this upper bound can be very loose when $\lam$ is close to $0$.
In fact, note that ${\rm UB}(\mathcal{I})$ is achieved by a {\em personalized} policy, but ${\rm OPT}(\mathcal{I})$ is defined over {\em non-personalized} policies.
Next, we construct a non-adaptive policy whose revenue is $\Omg\left(\frac 1k \right) \cdot \mathrm{UB}(\mathcal{I})$, which implies that UB approximates the optimum within a factor of $k$.


\subsection{Competitive Non-adaptive Policy}
The above upper bound motivates us to consider a simpler function $\tilde f(t_1,\dots, t_k;n_1,\dots,n_k) := {\rm Rev}(\mathcal{I}) / {\rm UB}(\mathcal{I})$ to serve as a surrogate for the original objective $f$. 
Unfortunately, $\tilde f$ is the ratio of two non-linear functions, and so the corresponding max-min problem is still challenging to solve directly.

We address this by {\em linearizing} both the numerator and denominator, thereby converting the max-min optimization to a linear program (LP).
We will show that the above sequence of reductions loses only a factor of $k$ (see Appendix \ref{apdx:non_adap}). 
We derive our robust non-adaptive policy by finding a closed-form solution to the final LP.}
{\neww \bdefn[Robust Policy]\label{def:non_adap}
Given any price set $\mathcal{P}=\{p_1,\dots,p_k\}$, the {\em robust policy} ${\bf t}^\star_{\mathcal{P}} =(t^\star_j)_{j\in [k]}$ is given by 
\begin{align} \label{eqn:lp_characterization}
t_k^\star = \frac{1}{k - \sum_{j=1}^{k-1} \frac{p_{j+1}}{p_{j}}} \quad \quad \text{and}\quad \quad  t_{j}^\star = \left(1 - \frac{p_{j+1}}{p_{j}} \right) t_k^\star, \quad \forall j=1,\dots, k-1.
\end{align}
\edefn

% Given any price set $\mathcal{P}=\{p_1,\dots,p_k\}$, the robust non-adaptive policy ${\bf t}^\star_{\mathcal{P}}$ can be computed using the recursion in \cref{eqn:lp_characterization}. 
% For example, when price set is $\mathcal{P} = \left\{1, \frac{2}{3}, \frac{1}{3}\right\}$, the robust non-adaptive policy ${\bf t}^\star_{\mathcal{P}}$ is  ${\bf t}^\star_{\mathcal{P}} = \left\{0, \frac{3}{11}, \frac{5}{11}\right\}$.
% For the uniform price set, the factor $1 - \frac{p_{i+1}}{p_{i}}$ is decreasing, thus the increase in $t_{j}^*$ is decreasing. 
For example, when $\mathcal{P} = \left\{1,2^{-1},\dots,2^{-(k-1)}\right\}$, we have $t_k^\star = 2/(k + 1)$ and $t^\star_j = 1/(k+1)$ for $j=1,\dots,k-1$ .
In other words, the policy spends $1/(k+1)$ time on each of the first $(k-1)$ prices and $2/(k+1)$ time on the last. 
}
{\OKsu 
We show that this policy is $1/k$ competitive.


% \su{Titing: give interesting examples (say, uniform, geometric valuations?). Explain why such a sequence make intuitive sense for these instances}

\begin{theorem}[Competitive Non-adaptive Policy]\label{thm:non-adap}
Denote by $\mathcal{F}_{\mathcal{P}}$ the family of UDPM instances with price set $\mathcal{P}$.
Then, 
\begin{align}\label{eqn:122723}
{\rm CR}({\bf t}^\star_{\mathcal{P}}, \mathcal{F}_{\mathcal{P}})\ge \frac{1}{k - \sum_{j=1}^{k-1} \frac {p_{j+1}}{p_j}} \ge \frac 1k.
\end{align}
% \tdtt{$p_{k+1}$ is a typo? Yes, it's a typo. It should be $p_{j + 1}$}
\end{theorem}

As a by-product, Theorem \ref{thm:non-adap} implies a bound on the adaptivity gap.
In fact, let $\Pi_{\rm NA}$ be the class of non-adaptive detail-free policies, and $\Pi$ be the class of (any) detail-free policies.
Let $\mathcal{F}_k$ be the set of UDPM instances with $k$ prices. 
For any instance $\cal I$, denote ${\rm OPT}_{\rm NA}(\mathcal{I}) = \sup_{X\in \Pi_{\rm NA}} {\rm Rev}(X, \mathcal{I})$.
Then,
\[{\rm Rev}({\bf t}^\star_{\cal P}, \cal I)\le {\rm OPT}_{\rm NA}(\cal I) \quad \text{and}\quad   {\rm UB}(\cal I)\ge {\rm OPT}(\mathcal{I}),\]
and therefore Theorem \ref{thm:non-adap} immediately implies the following.

\bcoro[Adaptivity Gap] For any $k\ge 1$ and $\mathcal{I} \in \mathcal{F}_k$, we have
${{\rm OPT}(\mathcal{I})}\le k\cdot {\rm OPT}_{\rm NA}(\mathcal{I}).$
\ecoro

% \su{explain in words.}
% Assuming $\{n_i\}_{i=1}^k$ is unknown in an instance.
% For a non-adaptive policy $\pi$, instead of computing the competitive ratio against the expected revenue of the optimal non-adaptive policy, we compute the competitive ratio against the upper bound ${\rm UB}(\mathcal{I})$. 
% Then, the worst-case competitive ratio can be reduced to a robust optimization: 

% \subsection{Upper Bound on the Competitive Ratio}
% We next show that no detail-free non-adaptive policy has a competitive ratio better than $1/k$.

% \begin{theorem}[Upper Bound on the Competitive Ratio]\label{thm:non_adap_upper} For any $\eps > 0, k \ge 1$ and detail-free non-adaptive policy ${\bf t}$, there is a UDPM instance $\cI_\eps\in \mathcal{F}_k$ such that \[{\rm Rev}({\bf t}, \mathcal{I}_\eps)\le \left(\frac 1k + \eps \right) {\rm OPT}(\mathcal{I}_\eps).\]
% \end{theorem}
% }
% {\neww To prove this, we construct for every $\bf t$ an instance $\cI_\eps$ wherein all customers have the same valuation, and therefore ${\rm OPT}(\cI_\eps) = {\rm UB}(\cI_\eps)$. 
% Furthermore, we choose $\lam$ to be small so that $\frac{{\rm Rev}(\cI_\eps)}{{\rm UB}(\cI_\eps)} \le  \frac{{\rm Rev}'(\cI_\eps)}{{\rm UB}'(\cI_\eps)} + \frac \eps2,$
% where ${\rm Rev}'$ and ${\rm UB}'$ are the linearized version of the revenue function and UB function (which we define  in Appendix \ref{apdx:UB}).
% Moreover, we choose the prices to be a geometric \xulie\ with a common ratio such that $\frac {{\rm Rev}'(\cI_\eps)}{{\rm UB'}(\cI_\eps)} \le \frac 1k + \frac \eps2$. 
% We defer the details to Appendix \ref{apdx:UB}.

% Discussion about other 1/k-competitive policy.

{\color{blue}
% Here we want to highlight that there exists multiple non-\adap\ policies that can achieve a $1/k$ competitive ratio. For example, a naive policy uses the decreasing price sequence each with a time interval $1/k$, which will also give a $1/k$ competitive ratio. Similarly, the robust stream policy outlined in \cref{sec:robust_stream} also maintains a competitive ratio of $1/k$. 
% However, 
Unlike these naive policies (NR and ND), our policy is parametrized by the prices. Notably, the competitive ratio of our policy significantly surpasses that of trivial algorithms in many cases, particularly for continuous price intervals. In the following subsection, we show that for continuous price intervals $[p_{\min}, p_{\max}]$, the competitive ratio of our policy converges to $\frac{1}{1 + \ln (\rho)}$ where $\rho = \frac{p_{\max}}{p_{\min}}$. In contrast, the competitive ratio of NR and ND converges to 0. This makes our policy substantially different from the naive policies. 
}




\iffalse To see the idea, recall that demand uncertainty is more difficult to handle when $\lam$ is small.
This motivates us to choose a sufficiently small $\lambda$ so that the linearization error is $O(\eps)$.
Moreover, we will choose $\cal P$ so that the competitive ratio is $\frac 1k+ O(\eps)$.
Then, we choose the valuation to be a Dirac \distr\ at a suitable price $p$ depending on the policy ${\bf t}$, and show that the fixed price policy yields at least $k$ times the revenue of ${\bf t}$.
Finally, we conclude by observing that ${\rm OPT}(\mathcal{I}_\eps)={\rm UB}(\mathcal{I}_\eps)$, since the valuation \distr\ is Dirac.
\fi
}

{\neww
\subsection{Competitive Ratio for Continuous Price Interval}
The bound in \cref{thm:non-adap}  assumes a finite price space.
Now we switch our attention to infinite price {\bf intervals}.  
To apply the results of the previous section, we consider a finite subset of prices in $\cal P$, given by a geometric grid. 
More precisely, \sps\ $\cal P=[a, b]$. For any $\eps > 0$, we define the {\em $\eps$-geometric grid} as 
\[\overline {\cal P}_\eps = \{a_\ell :=(1 + \eps)^\ell \mid \ell = 1,\dots, \lceil \log_{1+\eps}(b/a)\rceil\}.\]

We now analyze the competitive ratio of the robust policy (given in Definition \ref{def:non_adap}) on $\overline {\cal P}_\eps$. 
% {\neww \begin{proposition}
% [Competitive Ratio, Rounding-Based Policy]\label{thm:non-adap_lb2}
% Let $\mathcal{I}$ be a UDPM instance with a price set $\mathcal{P} = [p_{\min}, p_{\max}]$. Then,  
% \[\frac{{\rm Rev}({\bf t}^\star_{\overline{{\cal P}}_\eps}, \mathcal{I})}{{\rm UB}(\mathcal{I})} \ge \frac{1}{1 + \eps \log_{1+\eps}\frac{p_{\max}}{p_{\min}}}.\]
% \end{proposition}
% }
Note that  by restricting ourselves to the geometric grid, we lose a (multiplicative) factor of $(1 + \eps)$ in the revenue. Thus, 
\begin{align}\label{eqn:122923}
\frac{{\rm Rev}({\bf t}^\star_{\overline{\mathcal{P}}_\eps}, \mathcal{I})}{{\rm UB}(\mathcal{I})} \ge \frac 1{(1 + \epsilon)\lb(k - \sum_{i=1}^{k-1} \frac{p_{i+1}}{p_{i}}\rb)}= \frac 1{(1+\eps)(k-\frac {k-1}{1+\eps})}= \frac 1{1+\eps k}.
\end{align}
Note that $k= k(\eps)= \log_{1+\eps}(p_{\max}/p_{\min})$ and that $\eps/\ln (1+\eps)$ increases in $\eps$, so letting $\eps\rar 0^+$, we obtain
\[\eqref{eqn:122923}\ge \lim_{\eps\rar 0^+}\frac 1{1+ \eps \log_{1+\eps}\frac {p_{\max}}{p_{\min}}} = \frac 1{1+\ln \frac {p_{\max}}{p_{\min}}}.\]
We summarize the above as follows.

\begin{theorem}[Competitive Ratio for Price Intervals]\label{thm:conti_P}
For any UDPM \ins\ $\cal I$ with finite price set $\mathcal{P} = [p_{\min}, p_{\max}]$, the optimal non-adaptive policy  $X=(X_t)$ is given by 
\begin{align}\label{eqn:031424}
X_t = 
\begin{cases}
     p_{\max} \cdot e^{-t \lb(1 + \ln  \frac{p_{\max}}{p_{\min}}\rb)}, & \text{if  } 0 \le t \le 1 - \frac 1{1 + \ln  \frac{p_{\max}}{p_{\min}}}\\
    p_{\min}, & \text{if  }  1 - \frac{1}{1 + \ln  \frac{p_{\max}}{p_{\min}}} < t \le 1.
\end{cases}
\end{align}
Moreover, 
\[\frac{{\rm Rev}(X, \mathcal{I})}{{\rm UB}(\mathcal{I})} \ge \frac 1{1 + \ln\frac{p_{\max}}{p_{\min}}}.\]
\end{theorem}

}
% for the core set, and $p_{i+1}/p_{i} = 1/(1 + \epsilon)$ for $i \in [k-1]$. Plugging the expression of $k$ and $p_{i+1}/p_{i} $, then the competitive ratio on the core is
% \[
% \frac{1}{1 + \epsilon \log(p_1/p_k)/\log(1+\eps)} .
% \]
% Note that $\eps/\log(1+\eps)$ is increasing in $\epsilon$ and  therefore, the competitive ratio is at least,
% \[
% \frac{1}{1 + \eps\log(p_1/p_k)/\log(1+\eps)} \ge \frac{1}{1 + \log(p_1/p_k)}
% \]

% We obtain the following by applying the recursion in \cref{eqn:lp_characterization} to a geometric grid and letting the granularity approach zero.
% We defer the derivation of $X_t$ to Appendix \ref{proof:coro_continuous_price}.
  
\begin{figure}
\centering
 \includegraphics[width = 0.8\textwidth]{Figures/price_time.png}
 \caption{Robust non-adaptive policies with continuous price sets.}
\label{fig:price_time}
\end{figure}

{\OKsu 
We visualize the robust non-adaptive policies in \cref{fig:price_time}.
We observe that the price curves become steeper as $p_{\min}$ decreases and when $t$ approaches 1, the price reaches $p_{\min}$ and remains constant at $p_{\min}$ until the end of the horizon.
This is consistent with our intuition. 
In fact, when $p_{\min}$ is small, the ``opportunity cost'' of choosing the lowest price is relatively small. 
}

==> OR/regret_lower_bound.tex <==
{\bf Construction.}  \Sps\ the valuation \distr\ is supported on $\{p_H, p_L\}$.
Consider two \ins s $\mathcal{I}_0, \mathcal{I}_1$. 
They have the same number of customer at $p_L$. 
In $\mathcal{I}_0$ there is no buyers at $p_H$, but in $\mathcal{I}_1$ there is exactly {\bf one} buyer, referred to as the {\em special} buyer, in $p_H$.

{\bf Idea.} We will set $n\cdot p_L = O(1)$ and $p_H=1$, so that mishandling the special customer can cause $\Omg(1)$ (multiplicative) regret. Wlog normalize  the time horizon to be $1$. Then under instance $\mathcal{I}_1$, we need to spend $\Omg(1)$ time in $p_H$.

{\bf Proof outline.}

Step 1. Let $\tau$ be the number of times that we select $p_H$. If $\ho{E}_0 \tau$ is large, then bad under $\mathcal{I}_0$.

Step 2. If $\ho{E}_0[\tau]$ is small, then by Pinsker, $\ho{P}_0$ and  $\ho{P}_1$ are close. 
Specifically, for any event $A$, we have 
\[|\ho{P}_0 (A) - \ho{P}_1(A)| \le xx.\]
where RHS is a function of $\ho{E}_0 \tau$.

Step 3. Consider the event $A$ that we select  $p_H$ many times, which is a bad event under $\mathcal{I}_0$. 
\bitem 
\item If $\ho{P}_0(A)$ is large, then high regret under $\mathcal{I}_0$. 
\item If $\ho{P}_0(A)$ is small, i.e., $\ho{P}_0(A^c)$ is large, then $\ho{P}_1(A^c)$ is also large, i.e., we are likely to select $p_H$ very few times, then high is regret under $\mathcal{I}_1$. 
\eitem \qed

